BreakingBERT@IITK at SemEval-2021 Task 9 : Statement Verification and Evidence Finding with Tables

Recently, there has been an interest in factual verification and prediction over structured data like tables and graphs. To circumvent any false news incident, it is necessary to not only model and predict over structured data efficiently but also to explain those predictions. In this paper, as part of the SemEval-2021 Task 9, we tackle the problem of fact verification and evidence finding over tabular data. There are two subtasks. Given a table and a statement/fact, subtask A determines whether the statement is inferred from the tabular data, and subtask B determines which cells in the table provide evidence for the former subtask. We make a comparison of the baselines and state-of-the-art approaches over the given SemTabFact dataset. We also propose a novel approach CellBERT to solve evidence finding as a form of the Natural Language Inference task. We obtain a 3-way F1 score of 0.69 on subtask A and an F1 score of 0.65 on subtask B.

==> problem_delete.tex <==
\section{Problem Defintion}

%%Key points:
The problem statement is articulated around the following two related subtasks.

\subsection{Subtask A - Table Statement Support}
Given a statement/fact, some of which will be directly adapted from the linking text, and a table, determine whether the statement is supported by the information given in the table. In this classification problem, a statement is assigned one of the following labels:
\begin{enumerate}
\item[$\bullet$] \textbf{Fully Supported: } Statement is supported by data found within the table (denoted by 1).
\item[$\bullet$] \textbf{Refuted: } Statement is contradicted by table (denoted by 0).
\item[$\bullet$] \textbf{Unknown: } Not enough information in table to assess statement veracity (denoted by 2).

%%\item 2.2 Subtask B - Relevant Cell Selection

\end{enumerate}

%The first subtask consists of Table and Statement Support in which given a table and statement we have to determine whether the statement is supported by the table. In the second subtask Relevant Cell Selection we need to found which table cells form relevant evidence for the statement. Mathematically, the problem can be described as, given a table $\mathbb{T}$ that consists of cells $x_{ij}$ corresponding to row $r_{i}$ and column $c_{j}$, and a fact $\mathbb{F}$. We need to perform two subtasks as follows:



This can be denoted as a classification task, in which given $\{\mathbb{T},\mathbb{F}\}$, we need to perform the mapping to the output $y$ (corresponding to $\mathbb{F}$), where $y$ $\in \{0,1,2\}$.


\subsection{Subtask B - Relevant Cell Selection}
Given a statement and a table, find which table cells
form relevant evidence for the statement (if any).
A table cell is evidence for a statement if it helps
support or refute a part of the statement:

% \begin{figure}
% \centering
% \begin{subfigure}[h]{0.495\textwidth}
% \includegraphics[width=\textwidth]{images/2.PNG}
% \label{figure:outputb}
% \caption{Example Subtask B output for the statement in bold in Figure 1(b)}
% \end{subfigure}

% \begin{subfigure}[h]{0.495\textwidth}
% \includegraphics[width=\textwidth]{images/4.PNG}
% \caption{Example Subtask A output }
% \label{figure:statementb}
% \end{subfigure}
% \caption{Example Table and output for Subtask A \& B}
% \label{figure:completefig1}
% \end{figure}

\begin{enumerate}
\item[$\bullet$] \textbf{Relevant: }  the cell must be included. Denoted by 1.
% \item[$\bullet$] \textbf{Ambiguous: } the cell is allowed to be either included or not included. Denoted by 0.
\item[$\bullet$] \textbf{Irrelevant: } the cell must not be included. Denoted by 0.
\end{enumerate}

Mathematically, each cell $x_{ij} \in \mathbb{T}$, each $x_{ij}$ needs to be mapped to a value $y$ $\in$ $\{0,1\}$ for the corresponding $\mathbb{F}$.

We have also provided a sample output for our task in Table
\begin{table}[h!]
\begin{center}
\begin{tabular}{|p{2.8cm}|p{2cm}|p{1.5cm}|} 
\hline 
\textbf{Body Sensation}& \cellcolor[blue]{15}\textbf{hi} &\textbf{Pleasant}\\ 
\hline 
number & museum  & lovely  \\ 
\hline 
palpitation & shop  & happiness \\ 
\hline
heartbeat &boat  & Joyous   \\ \hline 
\end{tabular} 
\end{center}

\vspace{0.2cm}



\begin{tabular}{ p{5.5cm}p{2cm}} 
\textbf{Statement} & \textbf{Label} \\  
Palpitation is a bodily sensation & Supported \\ 
Joyous and boat have same strength & Unknown  \\ 
Lovely is an agoraphobic situation & Refuted \\ 
\end{tabular} 
\end{table}

\label{sec:length}
Table 1\footnote{based on example 0001.html with light edits}: A sample table and statement with correct results for subtask A and B. \textcolor{blue!65}{violet}: Relevant,  \textcolor{red!65}{red}: Irrelevant



% \subsection{Evaluation Measures}
% The evaluation of the results considers different
% strategies and metrics for Subtasks A and B in order to allow more fine-grained scores.
% % 

% \hspace{10pt}\textbf{Subtask A }The test set will be balanced between the three categories and the final ranking will be based on accuracy averaged across all three categories. There will
% be two evaluation methods. The first will be a standard precision/recall evaluation of a multi-class
% classification that evaluates whether each table was
% classified correctly as True / False / Unknown. This
% will test whether the classification algorithm understands cases where there is insufficient inform

